Multimodal Cross-Document Event Coreference Resolution Using Linear Semantic Transfer and Mixed-Modality Ensembles

Event coreference resolution (ECR) is the task of determining whether distinct mentions of events within a multi-document corpus are actually linked to the same underlying occurrence. Images of the events can help facilitate resolution when language is ambiguous. Here, we propose a multimodal cross-document event coreference resolution method that integrates visual and textual cues with a simple linear map between vision and language models. As existing ECR benchmark datasets rarely provide images for all event mentions, we augment the popular ECB+ dataset with event-centric images scraped from the internet and generated using image diffusion models. We establish three methods that incorporate images and text for coreference: 1) a standard fused model with finetuning, 2) a novel linear mapping method without finetuning and 3) an ensembling approach based on splitting mention pairs by semantic and discourse-level difficulty. We evaluate on 2 datasets: the augmented ECB+, and AIDA Phase 1. Our ensemble systems using cross-modal linear mapping establish an upper limit (91.9 CoNLL F1) on ECB+ ECR performance given the preprocessing assumptions used, and establish a novel baseline on AIDA Phase 1. Our results demonstrate the utility of multimodal information in ECR for certain challenging coreference problems, and highlight a need for more multimodal resources in the coreference resolution space.

==> mm_cdcr_fulltable.tex <==
\begin{table*}[!ht]
    \centering
    \tiny
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lllrrrrrrrrrrrrrrrrr@{}}
    \toprule
    &&& \multicolumn{3}{c}{MUC} && \multicolumn{3}{@{}c@{}}{$B^3$} & & \multicolumn{3}{c}{$CEAFe$} && CoNLL\\
    \cmidrule{4-6} \cmidrule{8-10} \cmidrule{12-14} \cmidrule{16-16}
    &&& R & P & $F_1$ && R & P & $F_1$ && R &P & $F_1$ && \multicolumn{1}{r}{$F_1$}  \\ 
   \midrule
        & \citet{held-etal-2021-focus} (no oracle) && 87.0  & 88.1 & 87.5 && 85.6 & 87.7 & 86.6 && 80.3 & 85.8 & 82.9 &&  85.7 \\
        & \citet{ahmed20232} (w/ oracle) && 93.1  & 88.5 & \textbf{90.8} && 93.6 & 80.7 & \textbf{86.7} && 82.0 & 87.5 & \textbf{84.7} &&  \textbf{87.4} \\
        \cdashline{1-20}
        %& \LLMFT~(w/ oracle)  && 89.8  & 87.6 & 88.7 && 90.7 & 80.2 & 85.1 && 82.5 & 85.1 & \textbf{83.8} &&  \textbf{85.9} \\
        %\cdashline{1-20}

        & \ViT-real\textrightarrow \LLM  && 3.6  & \textbf{92.1} & 6.9 && 46.2 & \textbf{99.7} & 63.1 && \textbf{87.1} & 40.2 & 55.1 &&  41.7 \\

        & \BEiT-real\textrightarrow \LLM  && 96.7  & 79.6 & 87.3 && 96.0 & 69.0 & 80.3 && 66.7 & 90.3 & 76.7 && 81.4  \\

        & \SWIN-real\textrightarrow \LLM  && 97.8  & 79.4 & 87.6 && 97.0 & 67.7 & 79.7 && 65.7 & 91.6 & 76.5 && 81.3 \\

        & \CLIP-real\textrightarrow \LLM  && 14.4  & 89.2 & 24.7 && 50.2 & 97.5 & 66.3 && 86.7 & 43.0 & 57.5 && 49.5 \\

        & \LLM \textrightarrow  \ViT-real && 98.9  & 79.6 & 88.2 && 97.7 & 67.8 & 80.1 && 66.1 & 93.5 & 77.5 && 81.9 \\

        & \LLM \textrightarrow  \BEiT-real  && \textbf{99.1}  & 79.6 & 88.3 && \textbf{97.9} & 67.7 & 80.0 && 65.9 & \textbf{93.7} & 77.4 && 81.9 \\
        
        & \LLM \textrightarrow  \SWIN-real    && 97.6  & 80.0 & 87.9 && 96.8 & 68.5 & 80.3 && 67.4 & 91.9 & 77.8 && 82.0 \\

        & \LLM \textrightarrow  \CLIP-real  && \textbf{99.1}  & 79.6 & 88.3 && \textbf{97.9} & 67.7 & 80.0 && 65.9 & \textbf{93.7} & 77.4 && 81.9 \\

        \cdashline{1-20}
        & \texttt{ViT}-gen $\oplus$ \texttt{LLM} && 80.9  & 89.7 & 85.1 && 85.4 & 86.9 & 86.1 && 85.5 & 76.5 & 80.7 && 84.0 \\

        & \texttt{BEiT}-gen $\oplus$ \texttt{LLM} && 75.9  & 89.7 & 82.2 && 82.5 & 87.5 & 84.9 && 85.3 & 71.9 & 78.1 &&  81.7 \\

        & \texttt{SWIN}-gen $\oplus$ \texttt{LLM}  && 75.7  & 90.7 & 82.5 && 82.3 & 88.0 & 85.1 && 86.6 & 72.1 & 78.7 && 82.1 \\

        & \texttt{CLIP}-gen $\oplus$ \texttt{LLM} && 95.4  & 84.0 & 89.3 && 95.3 & 75.4 & 84.2 && 75.9 & 90.7 & 82.6 && 85.4 \\
        
        \cdashline{1-20}

        & \ViT-gen\textrightarrow \LLM && 74.7  & 80.4 & 77.4 && 80.4 & 77.4 & 78.8 && 74.7 & 68.7 & 71.5 &&  75.9 \\

        & \BEiT-gen\textrightarrow \LLM  && 73.7  & 82.4 & 77.8 && 80.6 & 79.1 & 79.8 && 78.4 & 69.5 & 73.7 && 77.1 \\

        & \SWIN-gen\textrightarrow \LLM  && 78.5  & 80.6 & 79.5 && 83.0 & 76.5 & 79.6 && 74.6 & 72.3 & 73.4 &&  77.5 \\

        & \CLIP-gen\textrightarrow \LLM  && 83.4  & 82.7 & 83.0 && 86.8 & 77.9 & 82.1 && 75.9 & 76.7 & 76.3 &&  80.5 \\

        & \LLM \textrightarrow  \ViT-gen && 98.7  & 79.6 & 88.1 && 97.6 & 67.7 & 80.0 && 66.0 & 93.0 & 77.2 && 81.8 \\

        & \LLM \textrightarrow  \BEiT-gen  && \textbf{99.1}  & 79.6 & 88.3 && \textbf{97.9} & 67.7 & 80.0 && 65.9 & \textbf{93.7} & 77.4 && 81.9 \\

        & \LLM \textrightarrow  \SWIN-gen   && 99.0  & 79.6 & 88.2 && 97.8 & 67.8 & 80.1 && 66.0 & 93.5 & 77.4 &&  81.9 \\

        & \LLM \textrightarrow  \CLIP-gen  && \textbf{99.1}  & 79.6 & 88.3 && \textbf{97.9} & 67.7 & 80.0 && 65.9 & \textbf{93.7} & 77.4 && 81.9 \\
    \bottomrule
    \end{tabular}}
    \caption{MM-CDCR MUC, $B^3$, $CEAFe$ and CoNLL F1 results on ECB+ test set, using LLM only, {\tt Lin-Sem} (``\textrightarrow''), and domain-fused finetuned versions (``$\oplus$''). Cited works are previous benchmarks achieved on text-only CDCR. {\bf Bold} indicates the best performer on each metric (multiples indicate ties). ``-real'' indicates that the vision space was encoded with real images, while ``-gen'' indicates generated images.}
    \label{tab:mm_cdcr_full}
\end{table*}

